Lightweight Learning from Actuation-Space Demonstrations via Flow Matching for Whole-Body Soft Robotic Grasping

Robotic grasping under uncertainty remains a fundamental challenge due to its uncertain and contact-rich nature. Traditional rigid robotic hands, with limited degrees of freedom and compliance, rely on complex model-based and heavy feedback controllers to manage such interactions. Soft robots, by contrast, exhibit embodied mechanical intelligence: their underactuated structures and passive flexibility of their whole body, naturally accommodate uncertain contacts and enable adaptive behaviors. To harness this capability, we propose a lightweight actuation-space learning framework that infers distributional control representations for whole-body soft robotic grasping, directly from deterministic demonstrations using a flow matching model (Rectified Flow),without requiring dense sensing or heavy control loops. Using only 30 demonstrations (less than 8% of the reachable workspace), the learned policy achieves a 97.5% grasp success rate across the whole workspace, generalizes to grasped-object size variations of +-33%, and maintains stable performance when the robot's dynamic response is directly adjusted by scaling the execution time from 20% to 200%. These results demonstrate that actuation-space learning, by leveraging its passive redundant DOFs and flexibility, converts the body's mechanics into functional control intelligence and substantially reduces the burden on central controllers for this uncertain-rich task.

==> tex/algorithm.tex <==
%---------------- IEEE Python Style ----------------%
\lstdefinestyle{ieeepython}{
    language=Python,
    basicstyle=\footnotesize\ttfamily,   % compact and readable
    keywordstyle=\color{blue}\bfseries,
    commentstyle=\color{gray}\footnotesize\itshape,
    stringstyle=\color{red},
    numbers=left,
    numberstyle=\tiny,
    stepnumber=1,
    numbersep=5pt,
    frame=none,
    breaklines=true,
    showstringspaces=false,
    columns=flexible,
    xleftmargin=2ex
}



%---------------- Algorithm: Rectified Flow ----------------%
	%\vspace*{3.3cm} 
\begin{algorithm}[htbp]
\caption{\liudi{Rectified 
Flow for Learning Actions of SpiRob}}
\label{alg:cfm}
\begin{minipage}{0.8\linewidth} % 85% of column width
\begin{lstlisting}[style=ieeepython]
def train_step(batch):
    state, target_action = batch
    cond = state_encoder(state)
    tau = rand()         # normalized flow time 
    U0 = randn()                # Gaussian noise
    U1 = target_action          # expert control
    target_flow = U1 - U0
    U_tau = U0 + tau * target_flow
    pred_flow = model(U_tau, tau, cond)
    loss = mse(pred_flow, target_flow)
    return loss

def inference_step(state):
    """ open loop control, do once at the beginning"""
    cond = state_encoder(state)
    U = randn()
    for k in range(k_steps):
        tau = k / k_steps
        d_tau = 1 / k_steps
        pred_flow = model(U, tau, cond)
        U = U + pred_flow * d_tau
    return U
\end{lstlisting}
\end{minipage}
\end{algorithm}



